Root numbers and the parity problem

Let E be a one-parameter family of elliptic curves over a number field. It is natural to expect the average root number of the curves in the family to be zero. All known counterexamples to this folk conjecture occur for families obeying a certain degeneracy condition. We prove that the average root number is zero for a large class of families of elliptic curves of fairly general type. Furthermore, we show that any non-degenerate family E has average root number 0, provided that two classical arithmetical conjectures hold for two homogeneous polynomials with integral coefficients constructed explicitly in terms of E. The first such conjecture -- commonly associated with Chowla -- asserts the equidistribution of the parity of the number of primes dividing the integers represented by a polynomial. We prove the conjecture for homogeneous polynomials of degree 3. The second conjecture used states that any non-constant homogeneous polynomial yields to a square-free sieve. We sharpen the existing bounds on the known cases by a sieve refinement and a new approach combining height functions, sphere packings and sieve methods.

==> iby4extr.tex <==
% iby4extr.tex-- P.A.  MacKay -- July 12, 1997
% Pierre A. MacKay, Dept. of Classics, University of Washington
% mackay@cs.washington.edu
% ------------------------
% Provides traditional text-editor symbols for critical edition
% The control sequences follow Adobe naming conventions, to keep
% them from any likely conflict with plain.tex.
% I use \let\!=\dagger
% as a short and convenient way of getting at it
%
\def\braceleft{\char'333}
\def\braceright{\char'337}
\def\bracketleftbt{\char'363}
\def\bracketrightbt{\char'367}
\def\dagger{\char'375}
\def\dbldagger{\char'376}

\input version4


==> tlgsqq.tex <==
\def\sp_lenis{\char'076}%
\def\sp_asper{\char'074}%
\def\lenis_oxy{)'}%
\def\lenis_bary{)`}%
\def\lenis_peri{)=}%
\def\asper_oxy{('}%
\def\asper_bary{(`}%
\def\asper_peri{(=}%
\def\a_{a}%
\def\a_bary{a`}%
\def\a_aspr{a(}%
\def\a_len{a)}%
\def\a_isub{a|}%
\def\a_baryisub{a`|}%
\def\a_asprisub{a(|}%
\def\a_lenisub{a)|}%
\def\a_isub{a|}%
\def\a_oxy{a'}%
\def\a_asproxy{a('}%
\def\a_asprbary{a(`}%
\def\a_lenoxy{a)'}%
\def\a_lenbary{a)`}%
\def\a_oxyisub{a'|}%
\def\a_asproxyisub{a('|}%
\def\a_asprbaryisub{a(`|}%
\def\a_lenoxyisub{a)'|}%
\def\a_lenbaryisub{a)`|}%
\def\a_peri{a=}%
\def\a_asprperi{a(=}%
\def\a_lenperi{a)=}%
\def\a_periisub{a=|}%
\def\a_asprperiisub{a(=|}%
\def\a_lenperiisub{a)=|}%
\def\a_isub{a|}%
\def\e_{e}%
\def\e_bary{e`}%
\def\e_aspr{e(}%
\def\e_len{e)}%
\def\e_oxy{e'}%
\def\e_asproxy{e('}%
\def\e_asprbary{e(`}%
\def\e_lenoxy{e)'}%
\def\e_lenbary{e)`}%
\def\h_{h}%
\def\h_bary{h`}%
\def\h_aspr{h(}%
\def\h_isub{h|}%
\def\h_len{h)}%
\def\h_baryisub{h`|}%
\def\h_asprisub{h(|}%
\def\h_lenisub{h)|}%
\def\h_oxy{h'}%
\def\h_asproxy{h('}%
\def\h_asprbary{h(`}%
\def\h_lenoxy{h)'}%
\def\h_lenbary{h)`}%
\def\h_oxyisub{h'|}%
\def\h_asproxyisub{h('|}%
\def\h_asprbaryisub{h(`|}%
\def\h_lenoxyisub{h)'|}%
\def\h_lenbaryisub{h)`|}%
\def\h_peri{h=}%
\def\h_asprperi{h(=}%
\def\h_lenperi{h)=}%
\def\h_periisub{h=|}%
\def\h_asprperiisub{h(=|}%
\def\h_lenperiisub{h)=|}%
\def\h_isub{h|}%
\def\i_{i}%
\def\i_bary{i`}%
\def\i_aspr{i(}%
\def\i_len{i)}%
\def\i_oxy{i'}%
\def\i_asproxy{i('}%
\def\i_asprbary{i(`}%
\def\i_lenoxy{i)'}%
\def\i_lenbary{i)`}%
\def\i_peri{i=}%
\def\i_asprperi{i(=}%
\def\i_lenperi{i)=}%
\def\i_diaer{i+}%
\def\i_barydiaer{i+`}%
\def\i_oxydiaer{i+'}%
\def\i_peridiaer{i+=}%
\def\o_{o}%
\def\o_bary{o`}%
\def\o_aspr{o(}%
\def\o_len{o)}%
\def\o_oxy{o'}%
\def\o_asproxy{o('}%
\def\o_asprbary{o(`}%
\def\o_lenoxy{o)'}%
\def\o_lenbary{o)`}%
\def\u_{u}%
\def\u_bary{u`}%
\def\u_aspr{u(}%
\def\u_len{u)}%
\def\u_oxy{u'}%
\def\u_asproxy{u('}%
\def\u_asprbary{u(`}%
\def\u_lenoxy{u)'}%
\def\u_lenbary{u)`}%
\def\u_peri{u=}%
\def\u_asprperi{u(=}%
\def\u_lenperi{u)=}%
\def\u_diaer{u+}%
\def\u_barydiaer{u+`}%
\def\u_oxydiaer{u+'}%
\def\u_peridiaer{u+=}%
\def\w_{w}%
\def\w_bary{w`}%
\def\w_aspr{w(}%
\def\w_len{w)}%
\def\w_isub{w|}%
\def\w_baryisub{w`|}%
\def\w_asprisub{w(|}%
\def\w_lenisub{w)|}%
\def\w_oxy{w'}%
\def\w_asproxy{w('}%
\def\w_asprbary{w(`}%
\def\w_lenoxy{w)'}%
\def\w_lenbary{w)`}%
\def\w_oxyisub{w'|}%
\def\w_lenoxyisub{w)'|}%
\def\w_lenbaryisub{w)`|}%
\def\w_asproxyisub{w('|}%
\def\w_asprbaryisub{w(`|}%
\def\w_peri{w=}%
\def\w_asprperi{w(=}%
\def\w_lenperi{w)=}%
\def\w_periisub{w=|}%
\def\w_asprperiisub{w(=|}%
\def\w_lenperiisub{w)=|}%
\def\w_isub{w|}%



==> version4.tex <==
% version4.tex-- P.A.  MacKay -- July 15, 1997
% Pierre A. MacKay, Dept. of Classics, University of Washington
% mackay@cs.washington.edu
% ------------------------
\message{Ibycus Greek. Version 4. 15 July 1997}

